Plan-Driven Adaptive Bidding for First-Price Auctions with Budget Constraints under Nonstationarity

We study budget pacing in repeated first-price auctions when an advertiser's private-value distributions change over time and the stationary competing-bid distribution is unknown. We ask how a feasible expenditure plan should enter online bid shading, learning, and hard budget control. We establish a plan-to-performance decomposition for a plan-driven projected-dual policy. The policy uses any feasible expenditure plan as a soft target, learns an unknown stationary competing-bid CDF from thresholds revealed after each auction, and enforces the campaign budget on every sample path. Against a distribution-informed expected-budget fluid benchmark, the uniform-plan reward gap is $O(\sqrt T)+O(\mathcal W_T)$, where $\mathcal W_T$ measures heterogeneity in private-value distributions. With a supplied feasible plan, the global gap decomposes into a one-sided $O(\sqrt{T})$ fixed-plan execution term and a plan-mismatch term bounded by $(b/2a)PlanError$. The same analysis provides guarantees for strict and relaxed period-cap comparators, exact recovery of the global benchmark under a specific allowance vector, and separate lower bounds establishing the necessity of the temporal-heterogeneity and Plan Error terms. An upstream planner can translate forecasts or managerial priorities into a feasible spending trajectory, while the online controller adapts bids using realized thresholds and expenditures. The guarantee is modular: it evaluates the final normalized or projected plan through $PlanError$. A specific forecasting model can be linked to the guarantee by establishing how its primitive estimation errors propagate to this plan-quality metric.

==> major_revision/macros.tex <==
\RequirePackage{newtxtext}
\RequirePackage{newtxmath}
\RequirePackage{bm}

%\OneAndAHalfSpacedXI
%\OneAndAHalfSpacedXII % Current default line spacing
%%\DoubleSpacedXI
%%\DoubleSpacedXII

% Private macros here (check that there is no clash with the style)

% Natbib setup for author-number style
\usepackage{natbib}
 \bibpunct[, ]{(}{)}{,}{a}{}{,}%
 \def\bibfont{\small}%
 \def\bibsep{\smallskipamount}%
 \def\bibhang{24pt}%
 \def\newblock{\ }%
 \def\BIBand{and}%

\usepackage{amsmath}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{cleveref}
\usepackage{url}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage{array}

\newcommand{\E}{\mathbb{E}}
\newcommand{\Vpi}{V^{\pi}}
\newcommand{\VOPT}{V^{\mathrm{\scriptscriptstyle OPT}}}
\newcommand{\VLR}{V^{\mathrm{\scriptscriptstyle LR}}}
\newcommand{\VPLAN}{V_{\mathrm{plan}}^{\mathrm{\scriptscriptstyle OPT}}}
\newcommand{\PlanErr}{\mathcal{E}^{\mathrm{plan}}_T}
\newcommand{\brho}{\bm{\rho}}
\newcommand{\hrho}{\hat{\rho}}
\newcommand{\bhrho}{\bm{\hat{\rho}}}
\newcommand{\bepi}{\bm{\epsilon}}
\newcommand{\NPE}{\mathrm{NPE}}
\newcommand{\zR}{z^{\mathrm{\scriptscriptstyle R}}}
\newcommand{\gR}{g^{\mathrm{\scriptscriptstyle R}}}
\newcommand{\xR}{x^{\mathrm{\scriptscriptstyle R}}}
\newcommand{\muR}{\mu^{\mathrm{\scriptscriptstyle R}}}
\newcommand{\xb}{\bar{x}}
\newcommand{\dd}{\text{d}}

\definecolor{darkblue}{rgb}{0.05,0.25,0.60}
\definecolor{darkgreen}{rgb}{0,0.6,0}
\definecolor{darkred}{rgb}{0.75,0,0}
\definecolor{dbbpurple}{rgb}{0.5,0,0.9}
\theoremstyle{TH}
\newtheorem{thrm}{Theorem}[section]
\newtheorem{lemma}[thrm]{Lemma}
\newtheorem{prop}[thrm]{Proposition}
\newtheorem{coro}[thrm]{Corollary}

\theoremstyle{EX}
\newtheorem{remark}[thrm]{Remark}
 
%% Setup of the equation numbering system. Outcomment only one.
%% Preferred default is the first option.
\EquationsNumberedThrough    % Default: (1), (2), ...
%\EquationsNumberedBySection % (1.1), (1.2), ...

%% Setup of theorem styles. Outcomment only one.
%% Preferred default is the first option.
%\TheoremsNumberedThrough     % Preferred (Theorem 1, Lemma 1, Theorem 2)
%\TheoremsNumberedByChapter  % (Theorem 1.1, Lema 1.1, Theorem 1.2)
\ECRepeatTheorems  %  

